Video Labeling for Automatic Video Surveillance in Security Domains

Beyond traditional security methods, unmanned aerial vehicles (UAVs) have become an important surveillance tool used in security domains to collect the required annotated data. However, collecting annotated data from videos taken by UAVs efficiently, and using these data to build datasets that can be used for learning payoffs or adversary behaviors in game-theoretic approaches and security applications, is an under-explored research question. This paper presents VIOLA, a novel labeling application that includes (i) a workload distribution framework to efficiently gather human labels from videos in a secured manner; (ii) a software interface with features designed for labeling videos taken by UAVs in the domain of wildlife security. We also present the evolution of VIOLA and analyze how the changes made in the development process relate to the efficiency of labeling, including when seemingly obvious improvements did not lead to increased efficiency. VIOLA enables collecting massive amounts of data with detailed information from challenging security videos such as those collected aboard UAVs for wildlife security. VIOLA will lead to the development of new approaches that integrate deep learning for real-time detection and response.

==> BasicFramework.tex <==
\section{Basic Framework of \toolname} \label{basic-framework}
The main contribution of this paper is \toolname, an application we developed for labeling UAV videos in wildlife security domains. \toolname~includes a basic framework of work distribution and an easy-to-use interface for labelers. In this section, we introduce the basic framework of \toolname.

Our goal in labeling the challenging videos in wildlife security domain was first to keep the data secure, and second, to collect more usable labels to provide input for game-theoretic tools for security. In addition, we aim for getting exhaustive labels with high accuracy and consistency. To achieve these goals, we distribute the work among a small group of labelers in a secured manner, assign labelers to either provide labels or review others' labels and provide guidelines and training for the labelers.

\subsection{Distribution of Work} \label{distribution} 
To keep the data secure, instead of using AMT, we recruit a small group of labelers. For the historical videos we get from our collaborators, we recruited 13 labelers. They were given a username and password to access the labeling interface, and the images on the labeling interface could not be downloaded. 

In order to achieve label accuracy, we use a framework of label and review. The idea is simply that one person labels a video, and another person checks, or reviews, the labels of the first person. By checking the work of the labeler, the reviewer must agree or disagree with the original set of labels instead of creating their own. Upon disagreement, the reviewer could change the original labels. This was primarily chosen because it was a clean approach, leading to one set of final labels per video. This choice is described further in Sec. \ref{development}.

We use spreadsheets to share both assignments and completion progress with the team of labelers. The assignments were made once a week. We asked labelers to include the time it took for them to complete their assignment in order to help make future assignments more reasonable in terms of time commitment, and in order to track the efficiency and success of the application itself. If assignments were not completed in a week, the labelers were asked to provide an update and reason, and the labels were generally moved to the next week for that labeler to complete, or reassigned. Time commitment was agreed upon at the beginning of the semester. 

In addition, we split long videos into video segments to make it easier to make assignments respecting labelers' time commitments, and to finish extremely long videos more quickly. In addition, there were some videos that had long periods of nothingness, which were easier to ignore when the video was split. When we split videos, we made sure labelers knew what was happening in previous splits to ensure consistency by providing comments of labelers who are assigned to previous splits in the assignment spreadsheets.

\subsection{Guidelines and Training for Labelers} \label{guidelines}

In order to achieve accuracy and consistency of labels, we provide guidelines and training for the labelers. During the training, we show the labelers several examples of the videos and point out the features of interest. We provide them with general guidelines on how to start labeling a video, as below.

\paragraph{In general, the process for labeling should be:}
\begin{itemize}
	\item{Watch the video once all the way through and try to decide what you see.}
	\item{Once you have an idea of what is happening in the video by going through it, return to the beginning of the video and start labeling.}
	\item{Make and move bounding boxes.}
	\item{Send screenshots (including the percentage in the videos) if you need help.}
\end{itemize}

\paragraph{In general, the process for reviewing should be:}
\begin{itemize}
	\item{Refer to the guidelines and special circumstances directions, and any comments regarding the video.}
	\item{Go through the video, and use the eye button to check the original video and the labels.}
	\item{Move, create, or delete bounding boxes as necessary, either as you go or after watching the whole video. Try not to resize the bounding boxes unless they are much too big or too small. Only change the classification and add or delete boxes if certain, and please confirm with us if not.}
	\item{Send screenshots (including the percentage in the videos) if you need help.}
\end{itemize}
	
Since the UAV videos in our domain of interest are difficult to label, we also provide special instructions specific to these videos. For example, to distinguish between animals, humans, and plants or other objects, there were a few key clues: animals tended to be in herds, obviously shaped like animals, and/or significantly brighter than the rest of the scene, and humans tended to be moving. We also provided the following guidance for unusual videos:

\paragraph{Directions for special circumstances:}
 
\begin{itemize}
	\item{Only label when animals and humans are bright since the polarity changes occasionally}
	\item{If something is occluded completely: do not label}
	\item{If something is occluded a little but you can still see most features of them: label}
	\item{If something looks like it could be shaped like a human but never moves: do not label}
	\item{If something is cutoff halfway in/out of the frame: do not label}
	\item{If there are ``ghosts" (Fig. \ref{fig:ghost}) because you are ``in between" frames: do not label}
	\item{If you cannot recognize an individual (i.e., distinct poachers and animals): do not label}
\end{itemize}

The final instruction about distinct objects, was one of the more difficult instructions to follow because often, the aerial view and small targets made it difficult to tell if there were one or more animals. The movement instruction was also difficult, since with so few pixels on objects plus camera motion, it sometimes looked like objects were moving that were not. However, in these ambiguous cases, labelers were encouraged to ask for help. When there was still disagreement after discussion, we erred on the side of caution and only labeled certain objects.

\begin{figure}
	\includegraphics[width=0.3\textwidth]{figures_big_font/ghost1.png}
	\includegraphics[width=0.3\textwidth]{figures_big_font/ghost2.png}
	\includegraphics[width=0.3\textwidth]{figures_big_font/ghost3.png}
	\centering
	\caption{An example of a frame without ghosting (left), the next frame with ghosting (middle), and the next frame without ghosting (right). The middle frame is ``in between" the left and right frames.}
	\label{fig:ghost}
\end{figure}


==> Tool.tex <==
\section{User Interface of \toolname} \label{app}

The user interface of \toolname~was written in Java and Javascript, and hosted on a server through a cloud computing service so that it could be accessed using a URL from anywhere with an internet connection. 

Before labeling, labelers were asked to login to ensure data security (Fig. \ref{fig:menus1}). The first menu that appears after login (Fig. \ref{fig:menus2}) asks the labeler which mode they would like, whether they would like to label a new video or review a previous submission. 

Then, after choosing ``Label", the second menu (Fig. \ref{fig:menus3}) asks them to choose a video to label. It displays the chosen video and they are able to begin labeling. Fig. \ref{fig:example} is an example of the next screen used for labeling, also with a sample labeled frame that might be drawn at this stage. Along the top of the screen is an indication of the mode and the current video name, and along the bottom of the screen is a toolbar. First, in the bottom left corner, is a percentage indicating progress through the video. Then, there are four buttons used to navigate through the video. The two arrows move backwards or forwards, the play button advances frames at a rate of one frame per second, and the square stop button brings you back to the first frame of the video. The next button is the undo button, which removes the bounding boxes just drawn in the current frame, just in case they were too tiny to easily delete. Also to help with the nuisance of creating tiny boxes by accident while drawing a new bounding box or while moving existing bounding boxes, there is a filter on bounding box size. The trash can button deletes the labeler's progress and takes them back to the first menu after login (Fig. \ref{fig:menus2}). Otherwise, work is automatically saved after each change and re-loaded each time the browser is closed. The application asks for confirmation before deleting the labeler's progress, and undoing bounding boxes to prevent accidental loss of work. The checkmark button is used to submit the labeler's work, and is only pressed when the whole video is finished. Again, there is a confirmation screen to avoid accidentally submitting half of a video. The copy button and the slider will be described further in Sec. \ref{development}. The eye button allows the labeler to toggle whether or not to display the bounding boxes on the frame, which is often helpful during review to check that the labels were correct. Finally, the question mark button provides a help menu with a similar summary of the controls of the application (Fig. \ref{fig:help}). Notice the bounding boxes surrounding the animals in this video are colored red. Humans would be colored blue. This is also included in the help menu. 

To draw bounding boxes, the labeler can simply click and drag a box around the object of interest. Deleting a bounding box is done by pressing SHIFT and click, and selecting multiple bounding boxes is done by pressing CTRL and click. Selecting multiple bounding boxes allows the labeler to move multiple bounding boxes at once, and will be described further in Sec. \ref{development}. Finally, while navigating between frames the first time only, bounding boxes drawn in the current frame are moved to the next frame. It only happens the first time since it could otherwise add redundant bounding boxes or replace the bounding boxes originally added by the labeler.

If ``Review" is chosen in the first menu after login, the second menu also asks the labeler to choose a video to review, and then a third menu (Fig. \ref{fig:menus4}) asks them to choose a labeling submission to review. It finally displays the video with the labels from that particular submission, and they are able to begin reviewing the submission. The main difference between the labeling and review modes in the application is that the review mode displays an existing set of labels. The only other difference is that labels are not moved to the next frame in review mode. 

\begin{figure}
	\subfloat[][]{%
		\label{fig:menus1}%
		\includegraphics[width=0.45\textwidth]{figures/login.png}}%
	\subfloat[][]{%
		\label{fig:menus2}%
		\includegraphics[width=0.45\textwidth]{figures/first_menu.png}}\\
	\subfloat[][]{%
		\label{fig:menus3}%
		\includegraphics[width=0.45\textwidth]{figures/second_menu.png}}%
	\subfloat[][]{%
		\label{fig:menus4}%
		\includegraphics[width=0.45\textwidth]{figures/third_menu.png}}%
	\centering
	\caption{The menus to begin labeling. First, the labeler comes to the login screen (\ref{fig:menus1}), then the first menu, allowing the labeler to choose label or review mode (\ref{fig:menus2}). This is followed by the second menu, allowing the labeler to choose which video to label or review (\ref{fig:menus3}), and finally the third menu in review mode only, allowing the labeler to choose the labeling submission to check (\ref{fig:menus4}).}
	\label{fig:menus}
\end{figure}

\begin{figure}
	\includegraphics[width=0.45\textwidth]{figures/example1.png}
	\includegraphics[width=0.45\textwidth]{figures/example2.png}
	\centering
	\caption{An example of a frame (left) and labeled frame (right) in a video. This is the next screen displayed after all of the menus and allows the labeler to navigate through the video and manipulate or draw bounding boxes throughout.}
	\label{fig:example}
\end{figure}

\begin{figure}
	\includegraphics[width=0.6\textwidth]{figures/help.png}
	\centering
	\caption{Help screen displayed when the ? icon is selected, detailing the controls of the application.}
	\label{fig:help}
\end{figure}

